Using Machine Teaching to Boost Novices' Robot Teaching Skill

Recent evidence has shown that, contrary to expectations, it is difficult for users, especially novices, to teach robots tasks through LfD. This paper introduces a framework that leverages MT algorithms to train novices to become better teachers of robots, and verifies whether such teaching ability is retained beyond the period of training and generalises such that novices teach robots more effectively, even for skills for which training has not been received. A between-subjects study is reported, in which novice teachers are asked to teach simple motor skills to a robot. The results demonstrate that subjects that receive training show average 78.83% improvement in teaching ability (as measured by accuracy of the skill learnt by the robot), and average 63.69% improvement in the teaching of new skills not included as part of the training.

==> f_concept.tex <==
% Define block styles
\providecommand{\target}{\texttt{\textbackslash bthetad}}%
\providecommand{\sThetad}{\texttt{\textbackslash sThetad}}%
\providecommand{\ebtheta}{\texttt{\textbackslash ebtheta}}%
\providecommand{\Dd}     {\texttt{\textbackslash Dd}}%
\providecommand{\A}      {\texttt{\textbackslash A}}%
\providecommand{\bpi}      {\texttt{\textbackslash bpi}}%
\providecommand{\bx}      {\texttt{\textbackslash bx}}%
\providecommand{\D}      {\texttt{\textbackslash D}}%
\providecommand{\eD}     {\texttt{\textbackslash eD}}%
\providecommand{\eg}     {\texttt{\textbackslash eg}}%
\providecommand{\Acrlong}[1]{\texttt{\textbackslash Acrlong\{#1}\}}%
% \providecommand{\tasklearnt}{$\ebtheta\equiv$}%

\providecommand{\tasklearnt}{$\learnt\equiv\target$}%

% \providecommand{\tasklearnt}{$111$}%


%\tikzstyle{line} = [draw]
\tikzstyle{line} = [draw,->,>=stealth,thick]
\begin{tikzpicture}[node distance=.1675\linewidth, auto]
	\FPset{\imageheight}{0.075}
	%\draw [draw=none,fill=orange] (-0.055\linewidth,-0.125\linewidth) rectangle (0.260\linewidth,0.075\linewidth);
	%\draw [draw=none,fill=cyan  ] ( 0.260\linewidth,-0.100\linewidth) rectangle (0.360\linewidth,0.075\linewidth);
    % Place nodes
    \node [fill=white]                                                               (td) {\includegraphics[height=\imageheight\linewidth]{my_abb_td}};
	\node [fill=white,right of=td]                                                   (mt) {\includegraphics[height=\imageheight\linewidth]{abb_mt}};
	\node [fill=white,right of=mt]                                                   (ht) {\includegraphics[height=\imageheight\linewidth]{abb_ht}};
	\node [fill=white,right of=ht]                                                   (r)  {\includegraphics[height=\imageheight\linewidth]{abb_r}};
	\node [fill=white,right of=r ]                                                   (et) {\includegraphics[height=\imageheight\linewidth]{abb_tt}};
	\node [fill=white,xshift=-.020\linewidth,yshift=-.020\linewidth,right of=et]      {\includegraphics[height=\imageheight\linewidth]{my_abb_1}};
	\node [fill=white,xshift= .000\linewidth,yshift= .000\linewidth,right of=et] (tt) {\includegraphics[height=\imageheight\linewidth]{my_abb_1}};
	\node [fill=white,xshift= .020\linewidth,yshift= .020\linewidth,right of=et]      {\includegraphics[height=\imageheight\linewidth]{my_abb_1}};
	\node [yshift= 0.225\linewidth,xshift=.050\linewidth,below of=td]      {\parbox{.185\linewidth}{\raggedright\scriptsize Desired task}};
	\node [yshift=-0.225\linewidth,xshift=.050\linewidth,above of=td]      {\parbox{.185\linewidth}{\raggedright\scriptsize \eg pick object.}};
	\node [yshift= 0.225\linewidth,below of=mt]                            {\parbox{.185\linewidth}{\centering  \scriptsize \Acrlong{MT}}};
	\node [yshift= 0.225\linewidth,below of=ht]                            {\parbox{.185\linewidth}{\centering  \scriptsize Human teaches}};
	\node [yshift=-0.225\linewidth,above of=ht]                            {\parbox{.185\linewidth}{\centering  \scriptsize ... adapts teaching.}};
	\node [yshift= 0.225\linewidth,below of=r ]                            {\parbox{.185\linewidth}{\centering  \scriptsize Robot learns}};
	\node [yshift=-0.225\linewidth,above of=r ]                            {\parbox{.185\linewidth}{\centering  \scriptsize ... attempts task.}};
	\node [yshift= 0.225\linewidth,below of=et]                            {\parbox{.185\linewidth}{\centering  \scriptsize Taught task}};
	\node [yshift=-0.225\linewidth,above of=et]                            {\parbox{.185\linewidth}{\centering  \scriptsize ... \tasklearnt.}};
	\node [yshift=-0.265\linewidth,above of=mt] (api)                      {\parbox{ .25\linewidth}{\centering  \scriptsize Learning algorithm,\\control model}};
    % Draw edges
    \path [line] (td)  -- node[above] {\scriptsize$\target$}            (mt);
    \path [line] (mt)  -- node        {\scriptsize$\optiamldataset$}                 (ht);
	\path [line] (ht)  -- node[above] {\scriptsize$\D$}                  (r);
    \path [line] (r)   --                                     (et);
    \path [line] (api) -- node[xshift= .065\linewidth,left]  {\scriptsize$\A%(\cdot),
	\quad\bpi%(\bx,\cdot)
	$}           (mt);
	\path [line,transform canvas={xshift= 0.0725\linewidth}] (r)   |- (0.35\linewidth,-0.075\linewidth) node[xshift= .165\linewidth,yshift= .015\linewidth] {\scriptsize$\leanrerdataset$} --++ (ht);
	\path [line,transform canvas={yshift=-0.030\linewidth},red] (ht)  |- (0.75\linewidth,-0.080\linewidth) node[xshift=-.215\linewidth,yshift= .015\linewidth] {\scriptsize Generalises teaching skill to multiple tasks $\Model$} --++ (tt);
\end{tikzpicture}%


==> f_ui.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{img/exp1_ui.png}
    \caption{Simulation Platform User Interface: The interface displays a two-axis robotic arm fixed at the origin. The yellow marker and the blue arrow represent the robot's position and velocity, respectively. 
    % The green dashed line defines the action boundaries. 
    The dark green arrow shows the action applied by the user, and the light green arrows represent the \MT-based guidance.}
    \label{f:ui}
\end{figure}



==> hypotheses.tex <==
% The experiments are conducted in two scenarios: a simulation environment and a physical robot setup. 
% 基于MT提出的指导人类教学的框架是有效的。
To this end, the experimental hypotheses tested in this paper are: % was formulated to assess whether the MT-based guidance framework would enhance the quality of human teaching. The hypothesis are stated as:
\begin{enumerate}[label=$h_\arabic*$]
    % \item \label{h0}%\textbf{H1:} Teaching quality does not improve when humans are instructed by guidance derived from the principles of \MT.
    \item \label{h1}%\textbf{H1:} 
    Teaching quality improves when humans are instructed by guidance derived from the principles of \MT.
    \item \label{h2}%\textbf{H2:} 
    After guidance is removed, the improved teaching ability is retained.
    \item \label{h3}%\textbf{H3:} 
    The improved teaching ability learnt in one skill can be transferred to another skill.
    % \item The quality of the demonstration provided by the human teacher improves when they are instructed by guidance in the simulator.
    % \item The quality of the demonstration provided by the human teacher improves when they are instructed by guidance with a physical robot.
    %\item After guidance is removed, the improved teaching ability of human teachers on skills is retained.
    %\item The teaching abilities learnt by human teachers in one skill can be transferred to another skill.
\end{enumerate}
